Automated Extraction of Sentencing Decisions from Court Cases in the Hebrew Language

We present the task of Automated Punishment Extraction (APE) in sentencing decisions from criminal court cases in Hebrew. Addressing APE will enable the identification of sentencing patterns and constitute an important stepping stone for many follow up legal NLP applications in Hebrew, including the prediction of sentencing decisions. We curate a dataset of sexual assault sentencing decisions and a manually-annotated evaluation dataset, and implement rule-based and supervised models. We find that while supervised models can identify the sentence containing the punishment with good accuracy, rule-based approaches outperform them on the full APE task. We conclude by presenting a first analysis of sentencing patterns in our dataset and analyze common models' errors, indicating avenues for future work, such as distinguishing between probation and actual imprisonment punishment. We will make all our resources available upon request, including data, annotation, and first benchmark models.

==> sections/00_abstract.tex <==



==> tables/RB_ERR_table.tex <==
\begin{table*}[tb!]
\small
\centering
\begin{tabular}{p{2.5cm}p{3cm}p{10cm}}
\toprule
\textbf{Error (\% of examined cases)}             & \textbf{Example (English translation)}                                                                       & \textbf{Comments}      \\ \midrule
Probation (36\%) & \textit{In addition, 18 months probation.} &  Some sentences contain both the actual imprisonment and conditioned imprisonment [probation]. Since the probation sentencing has a more clearly defined structure and related indicative words, the algorithm learns the probation  structure as positive. Then, in cases where the actual imprisonment and the probation are separate, it erroneously chooses the probation instead of the actual imprisonment. \\\midrule
Reference to Previous Cases (46\%) &
\textit{The defendant was sentenced to 10 months probation with commitment to refrain from committing similar offense (2233/00)} &
Previous decisions regarding the defendant or previous cases that are brought to justify the current decision. \\\midrule
Party positions on desired punishment (13\%) &
\textit{Therefore, the prosecution requested to impose a punishment of a lengthy actual imprisonment, probation and a significant compensation to the victim.} &
Prosecution and defense positions on adequate punishment \\ \bottomrule
\end{tabular}
\caption{Error analysis of the rule-based learner shows that the most common mistake is probation sentences accounting for almost 50\% of the mistakes. Other than probation, errors are divided to references of past cases and positions of the parties on the desired punishment. These sentences are very similar in structure to those of the actual punishment, especially past cases which also confused the human taggers.}
\label{tab:ERR_RB}
\end{table*}

==> tables/RF_ERR_table.tex <==
\begin{table*}[tb!]
\small
\centering
\begin{tabular}{p{2.5cm}p{3cm}p{10cm}}
\toprule
\textbf{Error (\% of examined cases)}             & \textbf{Example}                                                                     & \textbf{Comments}      \\ \midrule  
Probation (65\%) & \textit{In addition, 18 months probation}.  & Similar to table \ref{tab:ERR_RB} \\ \midrule
Reference to Previous Cases  (18\%)   & \textit{The defendant was sentenced to 10 months probation with commitment to refrain from committing similar offense (2233/00)} & Similar to table \ref{tab:ERR_RB}                                                   \\ \midrule
Miscellaneous (17\%) & --                                               & This includes activation of probation, party positions on desired punishment, fines etc. \\ 
\bottomrule
\end{tabular}
\caption{Error analysis of the RF learner shows the highest error rate is caused by probation. This approach showed most bias towards probation sentences which account for over 50\% of the mistakes.  Second to probation are references to past cases. These errors are more similar to the rule-based than to the other supervised learner (SVM). Also these are the same cases that confused the human taggers.  In contrast to the other two models, the remaining mistakes of the RF are more random and cannot be categorized.}
\label{tab:Err_RF}
\end{table*}

==> tables/SVM_ERR_table.tex <==
\begin{table*}[tb!]
\small
\centering
\begin{tabular}{p{2.5cm}p{3cm}p{10cm}} \toprule
\textbf{Error (\% of examined cases)}             & \textbf{Example (English translation)}                                                                     & \textbf{Comments}      \\ \midrule
Probation (37.5\%)                                                                & \textit{In addition, 18 months probation.}                                                              & Some sentences contain both the actual imprisonment and conditioned imprisonment [probation]. Since the probation sentencing has a more clearly defined structure and related indicative words, the algorithm learns the probation structure as positive. Then, in cases where the actual imprisonment and the probation are separate, it erroneously chooses the probation instead of the actual imprisonment.\\\midrule
Fines (27.5\%)                                                                     & \textit{A fine of 5,000 NIS or 30 days imprisonment instead.} & Fines are usually followed by imprisonment substitution, if the fine is not paid. This also contains a form of "x duration imprisonment" however, it is not the punishment defined by the task.   \\ \midrule
Procedural Aspects of Imprisonment Sentencing (17.5\%)& \textit{Imprisonment starts on 31.}                              & This includes procedural arrangements rather than the  substantial announcement of imprisonment punishment.  The number ``31''. at the end of the sentence is probably part of a date, this is part of the problem in legal sentence extraction addressed by \cite{sanchez-2019-sentence} .  However this also happened with hours, and full dates.                                                                                                                                                       \\ \bottomrule
\end{tabular}
\caption{Error analysis of the SVM learner shows that most of the mistakes were made by choosing probation sentences. Other than probation, highest mistake rates are when the word for imprisonment is followed by numbers and that this model less relays on words such as "deciding", "sentencing","imposing" etc. In case of monetary fines imposed on the defendant, a human tagger would easily tag this as incorrect because of the word "fine", but the model was   confused by this, even though it did receive this as a feature.}
\label{tab:Err_svm}
\end{table*}

==> tables/mini_ratio_table.tex <==
\begin{table}[tb!]
\small
\centering
\resizebox{\columnwidth}{!}{  
\begin{tabular}{lccc}
\toprule
    Model &Sent F1 & APE  F1 & Avg Err (Months) \\ \midrule
\textbf{Rule-based}   & 0.7   & 0.64   & \textbf{5}   \\ 
\textbf{RF}  & \textbf{0.78}                                                                     & \textbf{0.65}                                                                         & 8.7                                                                    \\ 
\textbf{SVM} & 0.59                                                                     & 0.53                                                                          & 9.7                                                                      \\ \bottomrule
\end{tabular}
}
\caption{Full task evaluation, similar to Table ~\ref{tab:full_APE},  with additional annotations of punishment as appearing in the external summary added to to the legal document by the editorial team of the legal data base  ``mini ratio''. This once again demonstrates how improving the F1 measurement does not directly improve the average error in months} 
\label{tab:mini_ratio}
\end{table}
